Polynomial spline spaces of non-uniform bi-degree on T-meshes: Combinatorial bounds on the dimension

Polynomial splines are ubiquitous in the fields of computer aided geometric design and computational analysis. Splines on T-meshes, especially, have the potential to be incredibly versatile since local mesh adaptivity enables efficient modeling and approximation of local features. Meaningful use of such splines for modeling and approximation requires the construction of a suitable spanning set of linearly independent splines, and a theoretical understanding of the spline space dimension can be a useful tool when assessing possible approaches for building such splines. Here, we provide such a tool. Focusing on T-meshes, we study the dimension of the space of bivariate polynomial splines, and we discuss the general setting where local mesh adaptivity is combined with local polynomial degree adaptivity. The latter allows for the flexibility of choosing non-uniform bi-degrees for the splines, i.e., different bi-degrees on different faces of the T-mesh. In particular, approaching the problem using tools from homo-logical algebra, we generalize the framework and the discourse presented by Mourrain (2014) for uniform bi-degree splines. We derive combinatorial lower and upper bounds on the spline space dimension and subsequently outline sufficient conditions for the bounds to coincide.

==> ch_preliminaries_edge_groups.tex <==
\begin{definition}[Degree segments]\label{def:deg_seg}
	For interior edge $\edge \in \tmeshInteriorEH$ (resp. $\tmeshInteriorEV$), we define $\ids(\edge) \supseteq \edge$ as the maximal connected union of edges in $\tmeshInteriorEH$ (resp. $\tmeshInteriorEV$) such that for $\edge, \edge' \subseteq \ids$, $\pRing_{\edge} = \pRing_{\edge'}$. We will call $\ids(\edge)$ a \emph{degree segment}. A degree segment that does not intersect the boundary will be called an \emph{interior degree segment}.
\end{definition}
The sets of horizontal and vertical degree segments will be denoted $\DSH \equiv \DSH(\tmeshInteriorEH)$ and $\DSV \equiv \DSV(\tmeshInteriorEV)$, respectively, and we will define $\DS = \DSH \cup \DSV$.
Similarly, the sets of horizontal and vertical interior degree segments will be denoted $\IDSH \equiv \IDSH(\tmeshInteriorEH)$ and $\IDSV \equiv \IDSV(\tmeshInteriorEV)$, respectively, and we will define $\IDS = \IDSH \cup \IDSV$.
We define $\pRing_{\ids} = \pRing_{\edge}$ for any $\edge \subseteq \ids$.
\begin{definition}[Maximal segments]\label{def:ms}
	For a degree segment $\ids \in \DSH$, (resp. $\DSV$), we define $\ms(\ids) \supseteq \ids$ as the maximal connected union of degree segments in $\DSH$ (resp. $\DSV$); $\ms(\ids)$ will be called a \emph{maximal segment}.
\end{definition}
%The sets of horizontal and vertical maximal segments will be denoted $\MSH \equiv \MSH(\tmeshInteriorEH)$ and $\MSV \equiv \MSV(\tmeshInteriorEV)$, respectively, and we will define $\MS = \MSH \cup \MSV$.

\begin{definition}[Sub-maximal segments]\label{def:sms}
	For a maximal segment $\ms \in \MS$, order the degree segments forming $\ms$ along it in an ascending/descending fashion; let these ordered degree segments be denoted by $\ids_1, \dots, \ids_k$. Let $\sms^\ms_1, \dots, \sms^\ms_l$ form a partition of $\ms$ such that one of the following holds for all $i = 1, \dots, l$,
	\begin{equation*}
	\begin{split}
	&(A)~:~ \pRing_{\ids_{a_i}} \subseteq \dots \subseteq \pRing_{\ids_{b_i}}\;,\\
	&(B)~:~ \pRing_{\ids_{a_i}} \supseteq \dots \supseteq \pRing_{\ids_{b_i}}\;,\\
	&(C)~:~ \pRing_{\ids_{a_i}} \subseteq \dots \subseteq \pRing_{\ids_{c_i}} \supseteq \dots \supseteq \pRing_{\ids_{b_i}}\;,
	\end{split}
	\end{equation*}
	where $\sms^\ms_i = \bigcup_{j = a_{i}}^{b_{i}} \ids_j$.
	Then, we call $\sms^\ms_1, \dots, \sms^\ms_l$ the \emph{sub-maximal segments} forming $\ms$. While this partition need not be unique, we will assume that it is optimal, i.e., $l$ is the smallest possible integer for a given $\ms$.
\end{definition}
Note that we will omit the superscript of $\ms$ from $\sms^\ms$ where possible. The set of sub-maximal segments of $\ms$ will be denoted with $\SMS(\ms)$, while the set of all sub-maximal segments will be denoted with $\SMS \equiv \SMS(\tmesh)$. We will also denote the unique sub-maximal segment containing $\ids$ with $\sms(\ids)$; the unique maximal segment containing $\sms$  will be denoted with $\ms(\sms)$.

By the definition of the smoothness distribution, $\edge, \edge' \subset \ms \Rightarrow \bsmooth(\edge) = \bsmooth(\edge')$, and we therefore define $\bsmooth(\ms) = \bsmooth(\sms) = \bsmooth(\ids) = \bsmooth(\edge)$ for any $\edge \subseteq \ids \subseteq \sms \subseteq \ms$. Similarly, we define $\bideg{\ms} = \bideg{\sms} = \bideg{\ids} = \bideg{\edge}$ for any $\edge \subseteq \ids \subseteq \sms \subseteq \ms$. Finally, we define,
\begin{equation}
	\pRing_{\sms} = \sum_{\ids \subseteq \sms} \pRing_{\ids}\;,\qquad \pRing_{\sms, -\bideg{\sms}} = \sum_{\ids \subseteq \sms} \pRing_{\ids, -\bideg{\ids}}.
\end{equation}
Observe that by construction there exists $\edge \subset \sms$ such that $\pRing_{\sms} = \pRing_{\edge}$ and $\pRing_{\sms, -\bideg{\sms}} = \pRing_{\edge, -\bideg{\edge}}$.

\begin{remark}
	We will need to compute the dimensions of the vector spaces defined thus far in order to compute upper and lower bounds on the dimension of $\splSpace^\bsmooth_{\bdegree}$. This can be done using the approach outlined in Appendix \ref{app:vector_space_dimension}.
\end{remark}

